Iterative Bayesian Learning for Crowdsourced Regression

Crowdsourcing platforms emerged as popular venues for purchasing human intelligence at low cost for large volume of tasks. As many low-paid workers are prone to give noisy answers, a common practice is to add redundancy by assigning multiple workers to each task and then simply average out these answers. However, to fully harness the wisdom of the crowd, one needs to learn the heterogeneous quality of each worker. We resolve this fundamental challenge in crowdsourced regression tasks, i.e., the answer takes continuous labels, where identifying good or bad workers becomes much more non-trivial compared to a classification setting of discrete labels. In particular, we introduce a Bayesian iterative scheme and show that it provably achieves the optimal mean squared error. Our evaluations on synthetic and real-world datasets support our theoretical results and show the superiority of the proposed scheme.

==> additional_exp.tex <==
 % !TEX root =  main.tex


\section{PASCAL Visual Object Classes Datasets (More Results)}
\label{sec:detail_pascal}

\iffalse
In this section, we provide the experiment result demonstrating
the practical importance of the crowdsourced regression.
To do so, we investigate how the estimator, producing the training dataset,
 affect on the performance of convolutional neural network (CNN)
 for the object detection problem, which
 is a fundamental problem in the area of computer vision. 
% 
%Object detection task is the problem that finding target class objects in the given image. 
%Each image may contains more than one target class objects, 
%and detection algorithm needs to find all the target class objects (if any) 
%on input image by predicting bounding boxes, and classify which object is in that bounding boxes. 


%The PASCAL Visual Object Classes Homepage
%
%Pattern Analysis, Statistical modeling and computational learning

\noindent{\bf Generating datasets.}

We use {\MF VOC2007} and {\MF VOC2012} object detection datasets from \cite{pascal-voc-2007,pascal-voc-2012}, respectively. These datasets are one of the most widely used benchmark dataset for object detection. 
Both datasets contain twenty target class objects, with bounding box and class annotations. 
{\MF VOC2007} consists of $5,011$ images and $12,608$ labeled objects for 
train/val sets and $4,952$ images for test sets. 
{\MF VOC2012} train/val contains $11,540$ images and $27,450$ annotated objects. 
We trained detection model on two setting, 
which uses both VOC2007 and VOC2012 train/val as {\MF train data (07+12)} and 
trained only with VOC2007 train/val (07) and both models test on VOC2007 test set, 
which provides ground-truth labels.

BP,....


\noindent{\bf Performance evaluation.}

For the detection model, we use Single shot multibox detector (SSD) $300\times300$ model \cite{liu2016ssd}, 
Performance measure of detection is mean average precision 
which is usually used to benchmark for PASCAL VOC dataset, 
and decision of true positive or false positive of predicted bounding box is determined 
by whether intersection over union of ground-truth bounding box and predicted bounding box is larger than 0.5 or not.
Result ... table...

For the detection model, we use Single shot multibox detector (SSD) $300\times300$ model \cite{liu2016ssd}, 
which shows state-of-the-art performance on PASCAL VOC object detection dataset. 
It uses deep convolutional neural network as its based model and 
it is trained with input images and corresponding ground-truth class 
and bounding boxes annotations. 
In test phase, SSD outputs the bounding boxes and confidence of the object class 
inside the predicted bounding boxes given the query image. 
We use Caffe implementation of SSD \footnote{https://github.com/weiliu89/caffe/tree/ssd}, 
open-sourced by the authors. We follow the same training procedure such as, data augmentation,
and other hyper-parameter settings with the author's implementation for both 07+12 trainval and 07 trainval experiment,
except initial learning rate and train iteration for 07 trainval experiment. Initial learning rate and number of iterations 
are set as $10^{-5}$ and $60,000$ iterations, respectively.




The results of experiment shows in Table \ref{ssd-table}. We compare the performance of SSD  model trained with dataset removing noise by average method, naive method, belief propagation, oracle, and ground-truth label. 
\note{generation of dataset...} 
We apply this procedure on both 07+12 trainval set and 07 trainval set, and in both dataset, belief propagation achieves better accuracy compared to average and naive algorithm by maximum 5 mAP, and overlap between true positive boxes and ground-truth boxes are larger compared to average, naive algorithm. This indicates that SSD model trained with BP algorithm data less likely to miss the objects, and in the case of both models detect objects, it achieves higher bounding box location accuracy compared to average or naive method. These results verify experimentally that belief propagation method effectively reduces the noise in the crowdsourced label dataset compared to simple average or naive method, and benefit the the performance of the model that using those data.


The detection results example images are shown in Figure \ref{fig:ex1}. %,\ref{fig:ex2}, and \ref{fig:ex3}. 
In many examples, SSD model trained with dataset reducing noise
 by average methods most easily miss the objects or mis-localize the bounding boxes. 
 Naive, belief propagation, and oracle methods shows similar results, but belief propagation and 
oracle is usually slightly better than naive approaches in visual inspection.
In case of small objects, noise can hurt the performance more severely because even small noise can make the bounding box annotation mis-aligned with object very easily, and it is shown in the results Figure \ref{fig:ex1}, average method and naive method cannot detect the small object well compared to the oracle and belief propagation.

\begin{table}[t]
\caption{\textbf{PASCAL VOC2007 test detection results.} mAP and mean overlap results on VOC2007 test sets. Data: trained data model used. '07+12': VOC2007 trainval and VOC2012 trainval, '07': VOC2007 trainval. Overlap means average overlap of true positive bounding boxes with ground-truth bounding boxes}
\label{ssd-table}
\vskip 0.15in
\begin{center}
\begin{footnotesize}
\begin{sc}
\begin{tabular}{ccccc}
\hline
 \multirow{2}{*}{Data}  & \multirow{2}{*}{Algorithm} & {Mean Average }	 & \multirow{2}{*}{Overlap} \\
 & & { Precision} &\\
\hline
\multirow{5}{*}{\minitab[c]{VOC \\ 07+12}}	&Average    & 71.804 & 0.741 \\%/0.122 \\
					&Naive      &75.166 & 0.763 \\ %0.122 \\
					&BP & 75.936 & 0.772 \\ %/0.123\\
					&Oracle    & 76.051 & 0.774 \\ %/0.123\\
					&{Ground Truth}   & 77.789  & 0.784 \\ %/0.123        \\
\hline
\multirow{5}{*}{\minitab[c]{VOC \\ 07}} 	&Average & 62.698 & 0.711 \\ %/0.117 \\
				&Naive & XXX & XX \\ %/0.117 \\
				&BP & 67.520 & 0.736 \\ %/0.120\\
				&Oracle    &  67.548 & 0.736 \\ %/0.120\\
				&Ground Truth    & 69.474 & 0.746 \\ %/0.120       \\
\hline
\end{tabular}
\end{sc}
\end{footnotesize}
\end{center}
\vskip -0.1in
\end{table}

\fi





\begin{figure*}[t]
%\includegraphics[width=\textwidth]{figures/001037avg.png}
\subfigure{
\includegraphics[scale=0.5]{fig/vision/001037avg}%\caption{Average}
}
\subfigure{
\includegraphics[scale=0.5]{fig/vision/001037nav}% \caption{Naive}
}
\subfigure{
\includegraphics[scale=0.5]{fig/vision/001037bp}% \caption{Belief propagation}
}
\subfigure{
\includegraphics[scale=0.5]{fig/vision/001037ora}% \caption{Oracle}
}
%\includegraphics[width=\textwidth]{figures/intro_fig_2.png}
\caption{Detection examples on PASCAL VOC2007 test sets. Top left: Average, Top right: Naive, Bottom left: Belief Propagation, Bottom right: Oracles}\label{fig:ex2}
\end{figure*}






%\begin{figure*}[t]
%\centering
%%\includegraphics[width=\textwidth]{figures/001037avg.png}
%\subfigure{
%\includegraphics[scale=0.4]{figures/000547avg.png}%\caption{Average}
%}
%\subfigure{
%\includegraphics[scale=0.4]{figures/000547nav.png}% \caption{Naive}
%}
%\subfigure{
%\includegraphics[scale=0.4]{figures/000547bp.png}% \caption{Belief propagation}
%}
%\subfigure{
%\includegraphics[scale=0.4]{figures/000547ora.png}% \caption{Oracle}
%}
%%\includegraphics[width=\textwidth]{figures/intro_fig_2.png}
%\caption{Detection examples on PASCAL VOC2007 test sets. Top left: Average, Top right: Naive, Bottom left: Belief Propagation, Bottom right: Oracle}\label{fig:ex2}
%\end{figure*}

\begin{figure*}[t]
%\includegraphics[width=\textwidth]{figures/001037avg.png}
\subfigure{
\includegraphics[scale=0.5]{fig/vision/000196avg}%\caption{Average}
}
\subfigure{
\includegraphics[scale=0.5]{fig/vision/000196nav}% \caption{Naive}
}
\\
\subfigure{
\includegraphics[scale=0.5]{fig/vision/000196bp}% \caption{Belief propagation}
}
\subfigure{
\includegraphics[scale=0.5]{fig/vision/000196ora}% \caption{Oracle}
}
%\includegraphics[width=\textwidth]{figures/intro_fig_2.png}
\caption{Detection examples on PASCAL VOC2007 test sets. Top left: Average, Top right: Naive, Bottom left: Belief Propagation, Bottom right: Oracle}\label{fig:ex3}
\end{figure*}



  

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> proof_quanti.tex <==

% \eqref{eq:MSE_BP_bdd}, \eqref{eq:b_bdd},  \eqref{eq:2k_bound}, and \eqref{eq:concentration},
%since $\rho \in V$ and 
%$\tilde{\sigma}^2 \in \mathcal{S}^W$ are arbitrary and $\sigma^2$ is drawn from $\mathcal{S}^W$ uniformly at random.
% \eqref{eq:quantify}


%\begin{align*}
%& \EXP  \left[ \| \hat{\mu}^{{\MF BP} (k)}_i (A)  - \mu_i \|^2_2  \longmid \sigma^2_{M_i} \right] \\
%& \le \frac{d}{r+1}  \cdot \EXP \left[\frac{r+1}{\frac{1}{\tau^2} + \sum_{u \in M_i} \frac{1}{\sigma^2_u}   } \right]  \\
%&+ S^{\ell} \cdot \sqrt{8  \frac{d\sigma^6_{\max}}{\ell^3 \sigma^2_{\min}} \left(2  + \frac{d\sigma^6_{\max}}{\ell^3 \sigma^2_{\min}} \right)} \\
%& \times \left(4  \exp\left( -\frac{\varepsilon^2 r}{8(8\varepsilon+ 1) \sigma^2_{\max}}\right)  + \frac{3}{m}(\ell r)^{2k+1} \right) \;
%\end{align*}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End: 
